The Target-selection Pipeline for the Dark Energy Spectroscopic Instrument

In 2021 May, the Dark Energy Spectroscopic Instrument (DESI) began a 5 yr survey of approximately 50 million total extragalactic and Galactic targets. The primary DESI dark-time targets are emission line galaxies (ELGs), luminous red galaxies (LRGs) and quasars (QSOs). In bright time, DESI will focus on two surveys known as the Bright Galaxy Survey (BGS) and the Milky Way Survey (MWS). DESI also observes a selection of "secondary" targets for bespoke science goals. This paper gives an overview of the publicly available pipeline (desitarget) used to process targets for DESI observations. Highlights include details of the different DESI survey targeting phases, the targeting ID (TARGETID) used to define unique targets, the bitmasks used to indicate a particular type of target, the data model and structure of DESI targeting files, and examples of how to access and use the desitarget code base. This paper will also describe "supporting" DESI target classes, such as standard stars, sky locations, and random catalogs that mimic the angular selection function of DESI targets. The DESI target selection pipeline is complex and sizable; this paper attempts to summarize the most salient information required to understand and work with DESI targeting data.

==> DESI Target Selection Pipeline/table1.tex <==
\begin{deluxetable*}{cc}[t]
\tablecaption{Commands for importing DESI targeting bitmasks}\label{table:bitcmds}
\tablewidth{0pt}
\tablehead{
\colhead{Phase} & 
\colhead{Import command}
}
\startdata
 {\tt SV1} & {\tt from desitarget.sv1.sv1\_targetmask import desi\_mask, bgs\_mask, mws\_mask, scnd\_mask} \tablenotemark{a} \\
 {\tt SV2} & {\tt from desitarget.sv2.sv2\_targetmask import desi\_mask, bgs\_mask, mws\_mask, scnd\_mask} \\
 {\tt SV3} & {\tt from desitarget.sv3.sv3\_targetmask import desi\_mask, bgs\_mask, mws\_mask, scnd\_mask} \\
 {\tt main} & {\tt from desitarget.targetmask import desi\_mask, bgs\_mask, mws\_mask, scnd\_mask} \\
\enddata
\tablenotetext{a}{{\tt desi\_mask}, {\tt bgs\_mask}, {\tt mws\_mask} and {\tt scnd\_mask}, here, correspond to the different target type columns listed in Table~\ref{table:bitcols}. Any of the individual masks can be omitted from the command.}
\end{deluxetable*}

==> DESI Target Selection Pipeline/table10.tex <==
\begin{deluxetable*}{ccc}[t]
\tablecaption{Columns in the pixweight files}\label{table:pwcolumns}
\tablewidth{0pt}
\tablehead{
\colhead{Column Name} & 
\colhead{Python Format} &
\colhead{Description}
}
\startdata
{\tt HPXPIXEL}    & {\tt i4 } & HEALPixel integers at an input {\tt nside} (typically {\tt nside=256}). \\
{\tt FRACAREA}    & {\tt f4 } & Fraction of the HEALPixel with $\geq 1$ observation in any band.\tablenotemark{a} \\
{\tt STARDENS}    & {\tt f4 } & Density ($\mathrm{deg}^{-2}$) of stars in the HEALPixel from {\em Gaia} DR2 (see \S\ref{sec:pixweight}). \\
{\tt EBV}         & {\tt f4 } & Galactic dust extinction (E[B-V]).\tablenotemark{b} \\
{\tt PSFDEPTH\_X} & {\tt f4 } & $\frac{5}{\sqrt{{\tt PSFDEPTH\_X}}}$ gives the 5$\sigma$ flux-detection-limit in nanomaggies for a point source.\tablenotemark{b, c} \\
{\tt GALDEPTH\_X} & {\tt f4 } & As for {\tt PSFDEPTH\_X} but for a round, exponential galaxy of effective radius $0.45\arcsec$.\tablenotemark{b, c} \\
{\tt PSFSIZE\_X}  & {\tt f4 } & Weighted average PSF FWHM, in arcseconds.\tablenotemark{b, d} \\
{\tt FRACAREA\_X} & {\tt f4 } & Fraction of HEALPixel with $\geq 1$ observation in any band with MASKBITS=X.\tablenotemark{e} \\
{\tt \em{target name}} & {\tt f4 } & Target density in the HEALPixel for each target class bitname (see Table~\ref{table:tspapers}).\\
\enddata
\tablenotetext{a}{Derived from the {\tt NOBS\_G}, {\tt NOBS\_R}, {\tt NOBS\_Z} quantities in the random catalog.}
\tablenotetext{b}{This quantity is the median in the HEALPixel from the passed random catalog.}
\tablenotetext{c}{One each for optical and {\em WISE} bands (i.e.\ {\tt X} = {\tt G}, {\tt R}, {\tt Z}, {\tt W1}, {\tt W2}) where the {\em WISE} values are AB, not Vega.}
\tablenotetext{d}{One for each optical band (i.e.\ {\tt X} = {\tt G}, {\tt R}, {\tt Z}).}
\tablenotetext{e}{This is a bitwise OR, so, e.g., if X=7 then it's the fraction for $2^0\, |\, 2^1\, |\, 2^2$. {\tt MASKBITS} is described in the Legacy Surveys documentation at \url{https://www.legacysurvey.org/dr9/bitmasks/}.}
\end{deluxetable*}

==> DESI Target Selection Pipeline/table2.tex <==
\begin{deluxetable*}{ccccccc}[t]
\tablecaption{Relevant column names for DESI targeting bitmasks}\label{table:bitcols}
\tablewidth{0pt}
\tablehead{
\colhead{} & 
\colhead{} & 
\colhead{Primary Targets} & 
\colhead{} & 
\colhead{Secondary Targets} &  \\
\colhead{Survey Phase} & 
\colhead{Dark-time\tablenotemark{a}} & 
\colhead{BGS} &
\colhead{MWS} & 
\colhead{} & 
}
\startdata
 {\tt SV1} & SV1\_DESI\_TARGET & SV1\_BGS\_TARGET & SV1\_MWS\_TARGET & SV1\_SCND\_TARGET \\
 {\tt SV2} & SV2\_DESI\_TARGET & SV2\_BGS\_TARGET  & SV2\_MWS\_TARGET & SV2\_SCND\_TARGET  \\
 {\tt SV3} & SV3\_DESI\_TARGET & SV3\_BGS\_TARGET & SV3\_MWS\_TARGET & SV3\_SCND\_TARGET \\
 {\tt main} & DESI\_TARGET & BGS\_TARGET & MWS\_TARGET & SCND\_TARGET \\
\enddata
\tablenotetext{a}{Dark-time targets include LRGs, ELGs and QSOs.}
\end{deluxetable*}

==> DESI Target Selection Pipeline/table3.tex <==
\begin{deluxetable*}{lccr}[t]
\tablecaption{Publications that describe specific \desi\ science target classes}\label{table:tspapers}
\tablewidth{0pt}
\tablehead{
\colhead{Target selection class} & 
\colhead{Main Survey bit names\tablenotemark{a}} & 
\colhead{Brief description} &
\colhead{Selection detailed in}
}
\startdata
\sidehead{\em Dark-time targets}
 ~~~Luminous Red Galaxies & {\tt LRG} & LRG target & \citet{lrg} \\
 ~~~Emission Line Galaxies & {\tt ELG} & ELG target & \citet{elg} \\
                        & {\tt ELG\_LOP} & ELG at standard priority & \\
                        & {\tt ELG\_HIP} & ELG observed at the & \\
                        &                & priority of an LRG\tablenotemark{b} & \\
                        & {\tt ELG\_VLO} & Very-low-priority ``filler" ELG & \\
 ~~~Quasars & {\tt QSO} & Quasar target & \citet{qso} \\
\sidehead{\em Bright-time targets}
 ~~~Bright Galaxy Survey & {\tt BGS\_ANY} & Any BGS bit is set & \citet{bgs} \\
                      & {\tt BGS\_FAINT\tablenotemark{c}} & Faint BGS target & \\
                      & {\tt BGS\_BRIGHT} & Bright BGS target & \\
                      & {\tt BGS\_WISE} & AGN-like BGS target & \\              
                      & {\tt BGS\_FAINT\_HIP} & Faint BGS target prioritized & \\
                      &        & like a bright BGS target\tablenotemark{b} & \\
~~~Milky Way Survey & {\tt MWS\_ANY} & Any MWS bit is set & \citet{mws}\\
                  & {\tt MWS\_BROAD}\tablenotemark{d} & Magnitude-limited bulk sample &  \\
                  & {\tt MWS\_WD} & White dwarf &  \\
                  & {\tt MWS\_NEARBY} & Volume-limited $\sim$100\,pc sample &  \\
                  & {\tt MWS\_BHB} & Blue Horizontal Branch target &  \\
                  & {\tt MWS\_MAIN\_BLUE} & Magnitude-limited blue sample &  \\
                  & {\tt MWS\_MAIN\_RED} & Magnitude-limited red sample &  \\
\sidehead{\em Backup targets}
 ~~~~~~~~Part of the & {\tt BACKUP\_GIANT\_LOP}\tablenotemark{e}    & Candidate Giant Star & MWS et al.\ 2023 (in preparation) \\
  ~~~Milky Way Survey &                                             & observed at lower priority  &  \\
     & {\tt BACKUP\_GIANT}        & Candidate Giant Star &  \\
                          & {\tt BACKUP\_BRIGHT}   & Brighter backup target &  \\                    
                          & {\tt BACKUP\_FAINT}        & Fainter backup target &  \\
                          & {\tt BACKUP\_VERY\_FAINT}  & Even fainter backup target &  \\
\enddata
\tablenotetext{a}{Stored as bit-values in the {\tt DESI\_TARGET}, {\tt BGS\_TARGET} and {\tt MWS\_TARGET} columns. Bit-names can be converted to bit-values using the {\tt desi\_mask}, {\tt bgs\_mask} and {\tt mws\_mask} bitmasks (see \S\ref{sec:bitcols}).}
\tablenotetext{b}{Some targets with low observational priority are observed at higher priority to help characterize the survey selection function.}
\tablenotetext{c}{BGS bits other than {\tt BGS\_ANY} are stored in the {\tt BGS\_TARGET} column and {\tt bgs\_mask} bitmask.}
\tablenotetext{d}{MWS bits other than {\tt MWS\_ANY} are stored in the {\tt MWS\_TARGET} column and {\tt mws\_mask} bitmask.}
\tablenotetext{e}{BACKUP bits are stored in the {\tt MWS\_TARGET} column and {\tt mws\_mask} bitmask.}
\end{deluxetable*}

==> DESI Target Selection Pipeline/table4.tex <==
\begin{deluxetable*}{ccc}[t]
\tablecaption{Columns added to target files by the \dt\ pipeline}\label{table:tscolumns}
\tablewidth{0pt}
\tablehead{
\colhead{Column Name} & 
\colhead{Python Format} &
\colhead{Description}
}
\startdata
{\tt BRICK\_OBJID }   & {\tt i4 } & {\tt OBJID} from the Legacy Surveys sweep catalogs. \\
{\tt MORPHTYPE }     & {\tt U4 } & {\tt TYPE} from the Legacy Surveys sweep catalogs. \\
{\tt PHOTSYS }       & {\tt U1 } & `N' for {\em MzLS}/{\em BASS} photometric system, `S' for {\em DECaLS}.\tablenotemark{a} \\
{\tt TARGETID }      & {\tt i8 } &  See \S\ref{sec:targetid}. \\
{\tt DESI\_TARGET }   & {\tt i8 } & Column name differs for SV; see \S\ref{sec:bitcols}. \\
{\tt BGS\_TARGET }    & {\tt i8 } & Column name differs for SV; see \S\ref{sec:bitcols}. \\
{\tt MWS\_TARGET }    & {\tt i8 } & Column name differs for SV; see \S\ref{sec:bitcols}. \\
{\tt SCND\_TARGET }   & {\tt i8 } & Column name differs for SV; see \S\ref{sec:bitcols}. \\
{\tt SUBPRIORITY }   & {\tt f8 } &  Random number (0--1) used to break fiber-assignment ties.\\
{\tt OBSCONDITIONS } & {\tt i8 } & See \S\ref{sec:obscon}. \\
{\tt PRIORITY\_INIT } & {\tt i8 } & See E.\ Schlafly et al.\ 2023 (in preparation). \\
{\tt NUMOBS\_INIT }   & {\tt i8 } & See E.\ Schlafly et al.\ 2023 (in preparation). \\
{\tt HPXPIXEL }      & {\tt i8 } & The {\tt nside = 64} HEALPixel of the target.\tablenotemark{b} \\
\enddata
\tablenotetext{a}{{\em BASS}, {\em MzLS} and {\em DECaLS} are the individual surveys that comprise the \desi\ Legacy Imaging Surveys \citep[e.g.][]{Dey19}. The photometric system ({\tt bok} for {\em BASS}, {\tt mosaic} for {\em MzLS} and {\tt decam} for {\em DECaLS}) can be derived from the {\tt RELEASE} number according to \url{https://www.legacysurvey.org/release/}.}
\tablenotetext{b}{This {\tt nside} is stored in the file header as {\tt HPXNSIDE}.}
\end{deluxetable*}

==> DESI Target Selection Pipeline/table5.tex <==
\begin{deluxetable*}{crrrrrrr}[t]
\tablecaption{Densities (deg$^{-2}$) of principal Main Survey target classes in dark time}\label{table:targdensdark}
\tablewidth{0pt}
\tablehead{
\colhead{Bit name} & 
\colhead{\tt BGS\_ANY} & 
\colhead{\tt ELG} &
\colhead{\tt LRG} &
\colhead{\tt MWS\_ANY} &
\colhead{\tt QSO} &
\colhead{\tt STD\_BRIGHT\tablenotemark{a}} &
\colhead{\tt STD\_FAINT\tablenotemark{a}}
}
\startdata
{\tt BGS\_ANY}      & 79.8\tablenotemark{b} &    1.0\tablenotemark{c} &  78.4 &   0.5 &   0.9 &  0.0 &   0.0 \\
{\tt ELG}           &      & 2394.3 &   2.3 &   0.0 & 108.5 &  0.0 &   0.0 \\
{\tt LRG}           &      &        & 625.7 &   0.4 &   4.0 &  0.0 &   0.0 \\
{\tt MWS\_ANY}      &      &        &       & 119.0 &   7.6 & 51.9 & 104.2 \\
{\tt QSO}           &      &        &       &       & 319.8 &  0.0 &   0.0 \\
{\tt STD\_BRIGHT}   &      &        &       &       &       & 54.9 &  54.9 \\
{\tt STD\_FAINT}    &      &        &       &       &       &      & 107.2 \\
\enddata
\tablenotetext{a}{{\tt STD\_BRIGHT} and {\tt STD\_FAINT} are the main standard star classes intended for use in bright time and dark time, respectively (see \S{\ref{sec:standards}}).}
\tablenotetext{b}{On-diagonal elements represent the density for a target class, with areas derived using the {\tt desitarget} weight maps (see \S\ref{sec:pixweight}).}
\tablenotetext{c}{Off-diagonal elements represent the overlap in density between two target classes.}
\end{deluxetable*}

==> DESI Target Selection Pipeline/table6.tex <==
\begin{deluxetable*}{crrrrrrr}[t]
\tablecaption{Densities (deg$^{-2}$) of principal Main Survey target classes in bright time}\label{table:targdensbright}
\tablewidth{0pt}
\tablehead{
\colhead{Bit name} & 
\colhead{\tt BGS\_ANY} & 
\colhead{\tt ELG} &
\colhead{\tt LRG} &
\colhead{\tt MWS\_ANY} &
\colhead{\tt QSO} &
\colhead{\tt STD\_BRIGHT\tablenotemark{a}} &
\colhead{\tt STD\_FAINT\tablenotemark{a}}
}
\startdata
{\tt BGS\_ANY}      & 1389.7\tablenotemark{b} & 1.0\tablenotemark{c} &  78.4 &   0.6 &   0.9 &  0.0 &   0.0 \\
{\tt ELG}           &      &    1.0 &   0.4 &   0.0  &   0.0 &  0.0 &   0.0 \\
{\tt LRG}           &      &        &  78.8 &   0.4  &   0.3 &  0.0 &   0.0 \\
{\tt MWS\_ANY}      &      &        &       & 1910.5 &   7.6 & 51.9 & 104.2 \\
{\tt QSO}           &      &        &       &        &   8.0 &  0.0 &   0.0 \\
{\tt STD\_BRIGHT}   &      &        &       &        &       & 54.9 &  54.9 \\
{\tt STD\_FAINT}    &      &        &       &        &       &      & 107.2 \\
\enddata
\tablenotetext{a}{{\tt STD\_BRIGHT} ({\tt STD\_FAINT}) is the principal standard star class (see \S{\ref{sec:standards}}) intended for use in bright time (dark time).}
\tablenotetext{b}{On-diagonal elements represent the density for a target class, with areas derived using the {\tt desitarget} weight maps (see \S\ref{sec:pixweight}).}
\tablenotetext{c}{Off-diagonal elements represent the overlap in density between two target classes.}
\end{deluxetable*}

==> DESI Target Selection Pipeline/table7.tex <==
\begin{deluxetable}{c}[t]
\tablecaption{Columns that use {\em Gaia} EDR3 instead of DR2 when {\tt GAIASUB} is set in a file header. Columns are as for the Legacy Surveys sweep files.}\label{table:edr3}
\tablewidth{0pt}
\tablehead{
\colhead{Column name}
}
\startdata
{\tt PARALLAX} \\
{\tt PARALLAX\_IVAR} \\
{\tt PMRA} \\
{\tt PMRA\_IVAR} \\
{\tt PMDEC} \\
{\tt PMDEC\_IVAR} \\
{\tt GAIA\_DUPLICATED\_SOURCE} \\
{\tt GAIA\_ASTROMETRIC\_PARAMS\_SOLVED} \\
{\tt GAIA\_ASTROMETRIC\_SIGMA5D\_MAX} \\
{\tt GAIA\_ASTROMETRIC\_EXCESS\_NOISE} \\
\enddata

\end{deluxetable}

==> DESI Target Selection Pipeline/table8.tex <==
\begin{deluxetable*}{cc}[t]
\tablecaption{Target Selection for the {\tt STD\_BRIGHT} and {\tt STD\_FAINT}  target classes}\label{table:stdbright}
\tablewidth{0pt}
\tablehead{
\colhead{Reason for Selection} & 
\colhead{How Selection is Applied}
}
\startdata
Not masked &	{\tt MASKBITS}\tablenotemark{a,b} is not {\tt BRIGHT} or {\tt GALAXY} \\
Point-like & {\tt TYPE == "PSF"} \\
Isolated &	${\tt FRACFLUX\_X}\tablenotemark{c} < 0.01$ \\
Measured flux & ${\tt FLUX\_IVAR\_X} > 0$ \\
Observed &	${\tt NOBS\_X} > 0$ \\
Low fraction of masked pixels &	${\tt FRACMASKED\_X} < 0.6$ \\
Color of halo turnoff or bluer\tablenotemark{d}  &	$(r-z)<0.2$ AND $0.0 < (g-r) < 0.35$ \\
Reasonably bright in {\em Gaia}\tablenotemark{e} & $16 \leq {\tt PHOT\_G\_MEAN\_MAG} < 18$ \\
$Bp-Rp$ color is measured & ${\tt GAIA\_PHOT\_BP\_MEAN\_MAG} - {\tt GAIA\_PHOT\_RP\_MEAN\_MAG}$ is not {\tt NaN} \\
No astrometry issues &	${\tt GAIA\_ASTROMETRIC\_EXCESS\_NOISE} < 1$ AND \\
                     & ${\tt GAIA\_ASTROMETRIC\_PARAMS\_SOLVED} == 31$ \\
Proper motions are finite &	Neither {\tt PMRA} or {\tt PMDEC} is {\tt NaN} \\
Parallax smaller than 1\,mas & ${\tt PARALLAX} < 1$ \\
Proper motion larger than 2\,mas\,yr$^{-1}$ & $ \sqrt{{\tt PMRA}^2 + {\tt PMDEC}^2} > 2$ \\
Unique source in {\em Gaia} &	${\tt GAIA\_DUPLICATED\_SOURCE} == 0$ \\
\enddata
\tablenotetext{a}{Parameters that appear in this table are derived from the Legacy Surveys sweep files at \url{https://www.legacysurvey.org/dr9/files/\#sweep-catalogs-region-sweep}.}
\tablenotetext{b}{The Legacy Surveys {\tt MASKBITS} mask is described at \url{https://www.legacysurvey.org/dr9/bitmasks/}.}
\tablenotetext{c}{In this table, {\tt X} denotes that the criterion is applied for {\em all} bands from the Legacy Surveys ($g$, $r$ and $z$).}
\tablenotetext{d}{$g$, $r$, $z$ denote {\tt FLUX\_G}, {\tt FLUX\_R}, {\tt FLUX\_Z} converted to magnitudes and corrected for Galactic extinction.} 
\tablenotetext{e}{The only difference between the {\tt STD\_BRIGHT} and {\tt STD\_FAINT} target classes is that {\tt STD\_FAINT} extends across $16 \leq {\tt PHOT\_G\_MEAN\_MAG} < 19$.}
\end{deluxetable*}

==> DESI Target Selection Pipeline/table9.tex <==
\begin{deluxetable*}{cc}[t]
\tablecaption{Target Selection for the {\tt GAIA\_STD\_BRIGHT} and {\tt GAIA\_STD\_FAINT} target classes}\label{table:gaiastdbright}
\tablewidth{0pt}
\tablehead{
\colhead{Reason for Selection} & 
\colhead{How Selection is Applied}
}
\startdata
Point-like & ${\tt GAIA\_ASTROMETRIC\_EXCESS\_NOISE} < 10^{0.5}$  \\
Isolated &	No other {\em Gaia} source within 3.5\arcsec \\
Color of halo turnoff or bluer\tablenotemark{a} & $0.2 < (Bp - Rp) < 0.9$ AND \\
           & $(G - Bp) > -0.5(Bp - Rp)$ AND \\
           & $(G - Bp) < 0.3-0.5(Bp - Rp)$  \\
Reasonably bright in {\em Gaia}\tablenotemark{b} & $16 \leq {\tt PHOT\_G\_MEAN\_MAG} < 18$ \\
$Bp-Rp$ color is measured & ${\tt GAIA\_PHOT\_BP\_MEAN\_MAG} - {\tt GAIA\_PHOT\_RP\_MEAN\_MAG}$ is not {\tt NaN} \\
No astrometry issues &	${\tt GAIA\_ASTROMETRIC\_EXCESS\_NOISE} < 1$ AND \\
                     & ${\tt GAIA\_ASTROMETRIC\_PARAMS\_SOLVED} == 31$ \\
Proper motions are finite &	Neither {\tt PMRA} or {\tt PMDEC} is {\tt NaN} \\
Parallax smaller than 1\,mas & ${\tt PARALLAX} < 1$ \\
Proper motion larger than 2\,mas\,yr$^{-1}$ & $ \sqrt{{\tt PMRA}^2 + {\tt PMDEC}^2} > 2$ \\
Unique source in {\em Gaia} &	${\tt GAIA\_DUPLICATED\_SOURCE} == 0$ \\
\enddata
\tablenotetext{a}{In this table, $Bp$, $G$, $Rp$ denote versions of {\tt GAIA\_PHOT\_BP\_MEAN\_MAG}, {\tt GAIA\_PHOT\_G\_MEAN\_MAG}, {\tt GAIA\_PHOT\_RP\_MEAN\_MAG} that have been corrected for Galactic extinction using the prescription in Table 1 of \citet{Bab18}.}
\tablenotetext{b}{The only difference between the {\tt GAIA\_STD\_BRIGHT} and {\tt GAIA\_STD\_FAINT} target classes is that {\tt GAIA\_STD\_FAINT} extends across $16 \leq {\tt PHOT\_G\_MEAN\_MAG} < 19$.}
\end{deluxetable*}
